Efficient Verification and Falsification of ReLU Neural Barrier Certificates

Barrier certificates play an important role in verifying the safety of continuous-time systems, including autonomous driving, robotic manipulators and other critical applications. Recently, ReLU neural barrier certificates -- barrier certificates represented by the ReLU neural networks -- have attracted significant attention in the safe control community due to their promising performance. However, because of the approximate nature of neural networks, rigorous verification methods are required to ensure the correctness of these certificates. This paper presents a necessary and sufficient condition for verifying the correctness of ReLU neural barrier certificates. The proposed condition can be encoded as either an Satisfiability Modulo Theories (SMT) or optimization problem, enabling both verification and falsification. To the best of our knowledge, this is the first approach capable of falsifying ReLU neural barrier certificates. Numerical experiments demonstrate the validity and effectiveness of the proposed method in both verifying and falsifying such certificates.

==> necessary_controller.tex <==
\section{Necessary Criterion for the Existence of Locally Lipschitz Controller}
\begin{theorem}
    For the control affine system 
    \begin{equation}
    \label{control affine system}
        \dot{\bm{x}} = \bm{f}(\bm{x}) + \bm{g}(\bm{x}) \bm{u},
    \end{equation}


if there exists a locally lipschitz controller $\bm{u}(\bm{x}) \in \mathcal{U} \triangleq \{\bm{u}: \bm{A}_u \bm{u}\leq \bm{d}_u\}$ such that the $\mathcal{C}$ is positively invariant for the system \eqref{control affine system}, then the following nonlinear programming has non-negative optimal value for each valid region  $\mathcal{X}_i$. 

\begin{equation}   
                 \label{eq: controller nonlinear verification}
\begin{split}
     &\min_{\bm{x}, \bm{\mu}} \bm{w}_i^\top (\bm{f}(\bm{x})+\bm{d}_u^\top \bm{\mu})  \\
     \text{s.t.}~& \begin{cases}
              \bm{w}_i^\top \bm{x} + b_i=0,\\
         \bm{A}_i\bm{x} \leq \bm{d}_i,\\
         \bm{\mu}^\top \bm{A}_u = \bm{g}(\bm{x})
     \end{cases}
    \end{split}
\end{equation}
\end{theorem}

==> rebuttal.tex <==
We sincerely thank all reviewers for their careful reading and valuable comments. Due to space limitations, we primarily address the comments of Reviewer ZQaF to clarify certain misunderstandings.

Response to Reviewer ZQaF

1. We note that the condition in Thm.2—requiring Eq.(8) to hold for each valid linear region—is **both sufficient and necessary** to ensure the positive invariance of the 0-superlevel set of a CPLF. A detailed and rigorous proof has been provided in the appendix.

2. Our boundary propagation algorithm is fundamentally different from that of Zhang et al.(2024). It is derived directly from Thm.2 and requires identifying all **valid linear regions**. In contrast, Zhang et al.(2024) enumerate all **linear regions intersecting the boundary and their combinations**, which typically yields a larger set. Moreover, our algorithm includes a **valid test**, while theirs does not.

3. Fig. 3(a) illustrates the valid linear regions (the “hyperplanes” you mentioned), while Remark 3 discusses the **facets**. You might have mixed up these two concepts.

4. Both Zhang et al. (2023) and Zhang et al. (2024) share the same theoretical foundation and require enumerating all intersection combinations of linear regions intersecting the boundary, which can cause exponential computational growth (see Remark 2). When using the tool from Zhang et al.(2024), we observed that some intersection combinations of linear regions intersecting the boundary were not enumerated, compromising mathematical rigor. To ensure rigor and a fair comparison, we therefore primarily compare our approach against Zhang et al.(2023). Moreover, since Zhang et al.(2023, 2024) apply only a sufficient condition (see Remark 4), they may return “unknown” in some cases, whereas our approach can successfully verify (e.g., the Complex system in Tab.1). In addition, our method supports falsification, which theirs cannot.

5. We disagree with this comment. To the best of our knowledge, our work is the first to achieve **rigorous falsification**. Zhao et al.(2022) assume the derivative of ReLU is the Heaviside step function, which lacks mathematical rigor for falsification (see appendix). Zhang et al.(2023, 2024) use only sufficient conditions encoded as optimization problems (see Remark 4), making their methods unsuitable for falsification.

Response to Reviewers bGDP and CNRR

A statistical analysis of the computation times for each experiment will be included in the revised version.
 

==> rebuttal__history_.tex <==
Response to Reviewer ZQaF: 

1.Theorem 2 is derived from Proposition 2 , which demonstrates the points at the intersection of multiple regions must satisfy the condition (9) for each region.

\laode{
Your claim is not correct.
The condition in Thm.2 that for each valid linear region, eq (8) holds is sufficient and necessary for positive invariance of the 0-superlevel set of a CPLF, with rigorous proof provided in the appendix. 
}

2. The method used in Zhang et al 2024 did not check the validity of each region, and their termination condition of enumeration is different from ours as they did not check the duplicate of the regions. Moreover, their method must enumerate all the intersection of valid regions, which does not appear in our method.

\laode{
Your claim is not correct.
The boundary propagation algorithm is different from the method in Zhang et al, 2024 (abbv. Zhang): our algorithm is derived from Thm.2, requiring finding all valid linear regions, while Zhang enumerates all linear regions intersecting boundary, whose number is larger than ours; our algorithm requires \textbf{valid test} and \textbf{redundant constraints remove for linear regions}, while Zhang doesn't have.
}

3. For a 2-dimensional polyhedron, one line intersects it with at most 4 regions, as is shown in the dark blue region located in the upper right region of Fig.3 (a).

\laode{
When the system dimension is 2, the dimension of polyhedron $\mathcal{X}(\mathscr{C})$ is also 2, the boundary $\partial \mathcal{C}$, as a line in this polyhedron, intersects it with at most 4 \textbf{facets}.
}

4.\yiling{Both the methods in Zhang et al 2023,2024 enumerate region intersections, which is a key limitation of their methods. And they did not give improvement in Hinge Enumeration procedure. So we compare one of them to show the efficacy of our method. Moreover, Zhang et al 2024 reduced the regions intersecting the boundary, which greatly influences the time costs. To show the efficacy, we did not use this technique for verification.} 

\yiling{The time costs in Zhang et al 2023 are also different with ours. In their Darboux example with 2-64 NN architecture the time costs are only 2.02 while in our Arch3(both are 2-D examples) example their method costs up to 283.00. It shows the example and number of regions both affect the time costs.}

\yiling{Moreover, their method suffer from suboptimality while ours is not, as is shown in the Complex example with multiple "unknown" flag. This demonstrates our advantage over their method.}

\laode{

% When we used the method in Zhang24, it seems that their program has some bugs for enumerating all possible intersection combinations of linear regions, 
Both the methods in Zhang23, 24 requires enumerating all  intersection combinations of linear regions for verification, which may exponentially increase the computational burden  (see Remark 2). 
However,
When we used the method in Zhang24, it seems that their program may miss enumerating some  intersection combinations of linear regions, for the consideration of mathematical rigor and fair comparison, we compare our approach with Zhang23. 

% Nevertheless, Both the methods in Zhang23, 24 requires enumerating  region intersections, which is a key limitation of their methods. 
}
5. Zhang et al 2024 only encoded the verification into optimization, which suffers from suboptimality of nonlinear program solvers. Our method uses optimization to falsify and dReal to further verify, addressing the shortcomings of suboptimality. Zhao et al 2022 relied on the assumption the derivative of ReLU is heaviside step function, whose drawback is emphasized in our paper.

\laode{
Your claim is not correct. The method in Zhao et al 2022 relied on the assumption the derivative of ReLU is heaviside step function, which lacks mathematical rigor for  falsifying (see the appendix for details).
For Zhang et al, they could only use a sufficient condition for encoding the verification into optimization (see Remark 4), therefore their method cannot be used to falsify. 
}
Response to Reviewers bGDP and CNRR: 

% Since our algorithm doesn't rely on any random settings, the computation time won't vary to much for different runs.
We conducted each experiment five times, and the computation time exhibited minimal variation across runs. This statistical analysis will be included in the revised version. 










Response to Reviewer ZQaF:
1. Your claim is not correct. The condition in Thm.2 that for each valid linear region, eq (8) holds is sufficient and necessary for positive invariance of the 0-superlevel set of a CPLF, with rigorous proof provided in the appendix. 
2. Your claim is not correct. The boundary propagation algorithm is different from the method in Zhang et al, 2024 (abbv. Zhang): our algorithm is derived from Thm.2, requiring finding all valid linear regions, while Zhang enumerates all linear regions intersecting boundary, whose number is larger than ours; our algorithm requires \textbf{valid test} and \textbf{redundant constraints remove for linear regions}, while Zhang doesn't have.
3. When the system dimension is 2, the dimension of polyhedron $\mathcal{X}(\mathscr{C})$ is also 2, the boundary $\partial \mathcal{C}$, as a line in this polyhedron, intersects it with at most 4 \textbf{facets}.
4. Both the methods in Zhang23, 24 requires enumerating all  intersection combinations of linear regions for verification, which may exponentially increase the computational burden  (see Remark 2). However, When we used the method in Zhang24, it seems that their program may miss enumerating some  intersection combinations of linear regions, for the consideration of mathematical rigor and fair comparison, we compare our approach with Zhang23. 
5. Your claim is not correct. The method in Zhao et al 2022 relied on the assumption the derivative of ReLU is heaviside step function, which lacks mathematical rigor for  falsifying (see the appendix for details).
For Zhang et al, they could only use a sufficient condition for encoding the verification into optimization (see Remark 4), therefore their method cannot be used to falsify. 

Response to Reviewers bGDP and CNRR: 
We conducted each experiment five times, and the computation time exhibited minimal variation across runs. This statistical analysis will be included in the revised version. 



We sincerely thank all reviewers for their careful reading and valuable comments. Due to space limitations, we primarily address the comments of Reviewer ZQaF to clarify certain misunderstandings.

Response to Reviewer ZQaF:

1. We respectfully note that the condition in Thm. 2---requiring Eq. (8) to hold for each valid linear region---is **both sufficient and necessary** for the positive invariance of the 0-superlevel set of a CPLF. A rigorous proof is provided in the appendix.

2. We would like to clarify that our boundary propagation algorithm is fundamentally different that of Zhang et al.(2024). Our algorithm is derived directly from Thm. 2 and requires identifying all **valid** linear regions. In contrast, Zhang et al.(2024) enumerate all linear regions intersecting the boundary, which typically leads to a larger number of regions. Furthermore, our algorithm incorporates **valid test**, while the method in Zhang et al.(2024) does not.

3. For systems of dimension 2, the dimension of the polyhedron $\mathcal{X}(\mathscr{C})$ is also 2. Therefore, the boundary $\partial \mathcal{C}$, being a line in this polyhedron, intersects it with at most four **facets**(refer to the appendix for the definition).     


4. Both methods in Zhang et al.(2023) and Zhang et al.(2024) share the same theoretical foundation and  require enumerating all intersection combinations of linear regions for verification, which can result in exponential computational growth (see Remark 2). 
When using the tool proposed by Zhang et al.(2024), we observed that some intersection combinations might not have been enumerated. To ensure mathematical rigor and a fair comparison, we therefore primarily compare our approach against Zhang et al. (2023).
In addition, since both Zhang et al. (2023) and Zhang et al. (2024) only apply a sufficient condition for verification (see Remark 4), they may return “unknown” in certain cases, whereas our approach can successfully verify (e.g., the Complex system in Tab. 1). Moreover, our method is capable of falsification, while theirs is not.

% Besides, since both methods in Zhang et al.(2023) and Zhang et al.(2024) can only apply a sufficient condition for verification (see Remark 4), they may return ``unknown'' for verification, while our approach can successfully verify (e.g., the system Complex in Tab.1). Moreover, our method can falsify while they cannot.

5. We respectfully disagree with this comment. 
To the best of our knowledge, our work is the first method capable of **rigorous falsification**. 
Regarding Zhao et al.(2022), their approach assumes that the derivative of ReLU is the Heaviside step function, which lacks mathematical rigor for falsification (details are provided in the appendix). Zhang et al. (2023) and Zhang et al.(2024) employ only a sufficient condition to encode verification as a series of optimization problems (see Remark 4), rendering their method unsuitable for falsification.


---

Response to Reviewers bGDP and CNRR:

We conducted each experiment five times, and the computation time exhibited only minor variation across runs. This statistical analysis will be included in the revised version.


\yiling{-- revised version to limit the character} [9 characters left]

We sincerely thank all reviewers for their valuable comments. Due to space limitations, we primarily address the comments of Reviewer ZQaF to clarify misunderstandings.
Response to Reviewer ZQaF:
1. We note that the condition in Thm.2——requiring Eq.(8) to hold for each valid linear region——is **both sufficient and necessary** for the positive invariance of the 0-superlevel set of a CPLF.
2. We clarify that our boundary propagation algorithm is fundamentally different from the method in Zhang et al.(2024). Our algorithm is derived from Thm.2 and requires identifying all **valid** linear regions. In contrast, Zhang et al.(2024) enumerate all linear regions, which generally results in more regions than ours. Furthermore, our algorithm removes redundant linear regions, while theirs does not.
3. Since the polyhedron $\mathcal{X}(\mathscr{C}) \subset \mathbb{R}^2$ is two-dimensional, the boundary $\partial\mathcal{C}$, being a line within it, can intersect at most four facets.
4. Both methods in Zhang et al.(2023, 2024) share the same theoretical foundation and  require enumerating all intersection combinations of linear regions for verification, which can lead to exponential growth(see Remark 2). We attempted to reproduce the results using the code provided by Zhang et al.(2024). However, the released code could not be executed properly as some intersection combinations might not be enumerated. To ensure fairness, we compared against Zhang et al.(2023), which has similar design principles. Besides, since both methods in Zhang et al.(2023) and Zhang et al.(2024) can only apply a sufficient condition for verification (see Remark 4), they may return ``unknown'' for verification, while our approach can successfully verify (e.g., the system Complex in Tab.1. Moreover, our method can falsify while they cannot.
5. We respectfully disagree with this comment. 
Regarding Zhao et al(2022), their method relies on the assumption that the derivative of ReLU is the Heaviside step function, which lacks mathematical rigor for falsification (details are provided in the appendix). Zhang et al.(2024) can only apply a sufficient condition to encode verification into an optimization problem (see Remark 4), which makes their method unsuitable for falsification.
---
Response to Reviewers bGDP and CNRR:
We conducted each experiment five times, and the computation time exhibited only minor variation across runs. This statistical analysis will be included in the revised version.


\yiling{We indeed attempted to reproduce the results using the official implementation provided by Zhang et al.(2024). However, the released code could not be executed properly as some intersection combinations might not be enumerated. To ensure fairness, we therefore did not include unreliable results in the comparison table. Instead, we compared against Zhang et al.(2023), which has similar design principles. Besides, since both methods in Zhang et al.(2023) and Zhang et al.(2024) can only apply a sufficient condition for verification (see Remark 4), they may return ``unknown'' for verification, while our approach can successfully verify (e.g., the system Complex in Tab.1). Moreover, our method can falsify while they cannot.}





We sincerely thank all reviewers for their careful reading and valuable comments. Due to space limitations, we primarily address the comments of Reviewer ZQaF to clarify certain misunderstandings.

Response to Reviewer ZQaF:

1. We respectfully note that the condition in Thm.2---requiring Eq.(8) to hold for each valid linear region---is **both sufficient and necessary** for ensuring the positive invariance of the 0-superlevel set of a CPLF. A rigorous proof is provided in the appendix.

2. We would like to clarify that our boundary propagation algorithm is fundamentally different that of Zhang et al.(2024). Our algorithm is derived directly from Thm.2 and requires identifying all **valid** linear regions. In contrast, Zhang et al.(2024) enumerate all linear regions intersecting the boundary, which typically leads to a larger number of regions. Furthermore, our algorithm incorporates a **valid test**, whereas the method in Zhang et al.(2024) does not.

3. For systems of dimension 2, the dimension of the polyhedron $\mathcal{X}(\mathscr{C})$ is also 2. Therefore, the boundary $\partial \mathcal{C}$, being a line within this polyhedron, can intersect at most four **facets** (refer to the appendix for the definition).     


4. Both methods in Zhang et al.(2023) and Zhang et al.(2024) share the same theoretical foundation and  require enumerating all intersection combinations of linear regions that intersect the boundary for verification, which can result in exponential computational growth (see Remark 2). 
When using the tool from Zhang et al.(2024), we observed that some intersection combinations might not have been enumerated. To ensure mathematical rigor and a fair comparison, we therefore primarily compare our approach against Zhang et al. (2023).
In addition, since both Zhang et al. (2023) and Zhang et al. (2024) only apply a sufficient condition for verification (see Remark 4), they may return “unknown” in certain cases, whereas our approach can successfully verify (e.g., the Complex system in Tab. 1). Moreover, our method is capable of falsification, while theirs is not.

5. We respectfully disagree with this comment. 
To the best of our knowledge, our work is the first method capable of **rigorous falsification**. 
Regarding Zhao et al.(2022), their approach assumes that the derivative of ReLU is the Heaviside step function, which lacks mathematical rigor for falsification (details are provided in the appendix). Zhang et al. (2023) and Zhang et al.(2024) employ only a sufficient condition to encode verification as a series of optimization problems (see Remark 4), rendering their methods unsuitable for falsification.


---

Response to Reviewers bGDP and CNRR:

We conducted each experiment five times, and the computation time exhibited only minor variation across runs. This statistical analysis will be included in the revised version.


% 2500 version

We sincerely thank all reviewers for their careful reading and valuable comments. Due to space limitations, we primarily address the comments of Reviewer ZQaF to clarify certain misunderstandings.

Response to Reviewer ZQaF

1. We note that the condition in Thm.2—requiring Eq.(8) to hold for each valid linear region—is **both sufficient and necessary** to ensure the positive invariance of the 0-superlevel set of a CPLF. A rigorous proof is provided in the appendix.

2. Our boundary propagation algorithm is fundamentally different from that of Zhang et al.(2024). It is derived directly from Thm.2 and requires identifying all **valid** linear regions. In contrast, Zhang et al.(2024) enumerate all linear regions intersecting the boundary, which typically yields a larger set. Moreover, our algorithm includes a **valid test**, while theirs does not.

3. For 2D systems, the polyhedron $\mathcal{X}(\mathscr{C})$ is also two-dimensional. Hence, the boundary $\partial \mathcal{C}$, being a line within this polyhedron, can intersect at most four **facets** (see the appendix for the definition).

4. Both Zhang et al. (2023) and Zhang et al. (2024) share the same theoretical foundation and require enumerating all intersection combinations of linear regions intersecting the boundary for verification, which can cause exponential computational growth (see Remark 2). When using the tool from Zhang et al.(2024), we found some intersection combinations unenumerated. To ensure rigor and fairness, we therefore primarily compare our approach against Zhang et al.(2023). Moreover, since Zhang et al.(2023, 2024) apply only a sufficient condition (see Remark 4), they may return “unknown” in some cases, whereas our approach can successfully verify (e.g., the Complex system in Tab.1). In addition, our method supports falsification, which theirs cannot.

5. We disagree with this comment. To the best of our knowledge, our work is the first to achieve **rigorous falsification**. Zhao et al.(2022) assume the derivative of ReLU is the Heaviside step function, which lacks mathematical rigor for falsification (see appendix). Zhang et al.(2023, 2024) use only sufficient conditions encoded as optimization problems (see Remark 4), making their methods unsuitable for falsification.

Response to Reviewers bGDP and CNRR

Each experiment was run five times, and computation times showed only minor variation. This statistical analysis will be included in the revised version.





10/9 21:00


We sincerely thank all reviewers for their careful reading and valuable comments. Due to space limitations, we primarily address the comments of Reviewer ZQaF to clarify certain misunderstandings.

Response to Reviewer ZQaF

1. We note that the condition in Thm.2—requiring Eq.(8) to hold for each valid linear region—is **both sufficient and necessary** to ensure the positive invariance of the 0-superlevel set of a CPLF. A rigorous proof is provided in the appendix.

2. Our boundary propagation algorithm is fundamentally different from that of Zhang et al.(2024). It is derived directly from Thm.2 and requires identifying all **valid** linear regions. In contrast, Zhang et al.(2024) enumerate all linear regions intersecting the boundary, which typically yields a larger set. Moreover, our algorithm includes a **valid test**, while theirs does not.

3. Fig. 3(a) illustrates the valid linear regions (the “hyperplanes” you mentioned), while Remark 3 discusses the **facets**. You might have mixed up these two concepts.

4. Both Zhang et al. (2023) and Zhang et al. (2024) share the same theoretical foundation and require enumerating all intersection combinations of linear regions intersecting the boundary for verification, which can cause exponential computational growth (see Remark 2). When using the tool from Zhang et al.(2024), we observed that some intersection combinations were not enumerated, compromising mathematical rigor. To ensure rigor and a fair comparison, we therefore primarily compare our approach against Zhang et al.(2023). Moreover, since Zhang et al.(2023, 2024) apply only a sufficient condition (see Remark 4), they may return “unknown” in some cases, whereas our approach can successfully verify (e.g., the Complex system in Tab.1). In addition, our method supports falsification, which theirs cannot.

5. We disagree with this comment. To the best of our knowledge, our work is the first to achieve **rigorous falsification**. Zhao et al.(2022) assume the derivative of ReLU is the Heaviside step function, which lacks mathematical rigor for falsification (see appendix). Zhang et al.(2023, 2024) use only sufficient conditions encoded as optimization problems (see Remark 4), making their methods unsuitable for falsification.

Response to Reviewers bGDP and CNRR

==> related_work.tex <==
\subsection*{Related Work}
\label{related work}
% \color{blue}

\noindent\textbf{Inner-approximation analysis}
% Reachable sets are of interest in various contexts. 
% For example, they are essential to solve verification or control synthesis problems with respect to safety via ensuring that unsafe set is never reached or reachability properties via ensuring that a target set is eventually reached. 
% The exact computation of a reachable set is usually impossible, unless we deal with very specific and simple systems \cite{lafferriere2001symbolic}. Therefore, outer-approximations and inner-approximations of reachable sets are often computed in order to reason formally on the system. Many of the existing works focus on outer-approximations such as Taylor model methods \cite{makino2003taylor,chen2012taylor}, ellipsoids-based method \cite{kurzhanski2002ellipsoidal}, polytopes-based methods \cite{girard2006efficient,dreossi2016parallelotope}, zonotopes-based methods \cite{girard2005reachability,althoff2008reachability}, and level-sets based methods \cite{mitchell2003overapproximating}. In contrast, inner-approximations of reachable sets have received comparatively less attention than outer-approximations. 
The methods for inner-approximation computation are generally categorized into two main groups: constraint solving methods and set-propagation methods. Constraint solving methods avoid the explicit computation of reachable sets, but have to address a set of quantified constraints, which are generally constructed via Lyapunov functions \cite{branicky1998multiple}, occupation measures \cite{korda2013inner} and  equations relaxation \cite{xue2019inner,xue2022reach}. However, solving these quantified constraints is usually computationally intensive (except the case of polynomial constraints for which there exists advanced tools such as semi-definite programming). 

The set propagation method is an extension of traditional numerical methods for solving ODEs using set arithmetic rather than point arithmetic. 
% This method is simple and interesting. The major problem hindering its application is the propagation
% and accumulation of approximation errors over time. 
While this method is simple and interesting, a major challenge is the propagation and accumulation of approximation errors over time.
To ease this issue efficiently, various methods employing different representations have been developed. \cite{rwth2014under} presented a Taylor model backward flowpipe method that computes inner-approximations by representing them as the intersection of polynomial inequalities. However,  this approach relied on a computationally expensive interval constraint propagation technique to ensure the validity of the representation. In \cite{goubault2017forward}, an approach is proposed to compute interval inner-approximations of the projection of the reachable set onto the coordinate axes for autonomous nonlinear systems. This method is later extended to systems with uncertain inputs in \cite{goubault2019inner}. However, they cannot compute an inner-approximation of the entire reachable set, as studied in the present work. \cite{xue2016under} proposed a set-boundary reachability method which propagates the initial set's boundary to compute an polytopic inner-approximation of the reachable set.  However, it used computationally expensive interval constraint satisfaction techniques to compute a set of intervals which over-approximates the initial set's boundary. Recently, inspired by the computational procedure in \cite{xue2016under}, \cite{kochdumper2020computing} introduced  a promising method based on polynomial zonotopes to compute inner-approximations of reachable sets for systems with an initial set in interval form. The method presented in this work is also inspired by the in \cite{xue2016under}. 
%However, we propose an efficient \& accurate algorithm for refining the boundary of the initial set represented by zonotopes 
However, we propose efficient and accurate algorithms for extracting and refining the boundary of the initial set represented by zonotopes
and an adaptive strategy for contracting outer-approximations, facilitating the computation of non-conservative inner-approximations. 

\noindent\textbf{Splitting and tiling of zonotopes}
To mitigate wrapping effect \cite{neumaier1993wrapping} and enhance computed results, it is a common way to split a zonotope into smaller zonotopes during computation. 
%Although zonotopes are special convex polytope with centrally symmetric faces in all dimension, one can not straightforwardly apply traditional polytope splitting methods e.g. \cite{bajaj1996splitting,herrmann2008splitting} on zonotopes since the results after splitting via these approaches are still polytopes, not zonotopes. 
Despite zonotopes being special convex polytopes with centrally symmetric faces in all dimensions \cite{ziegler2012lectures}, traditional polytope splitting methods such as \cite{bajaj1996splitting,herrmann2008splitting} cannot be directly applied. The results obtained through these approaches are polytopes, not necessarily zonotopes.
In the works \cite{althoff2008reachability,wan2009numerical}, they split a zonotope by bisecting it along one of its generators. However, the sub-zonotopes split by this way often have overlap parts, resulting in loss of precision and heavy computation burden. Hence, there is a pressing need for methods that split a zonotope into non-overlapping sub-zonotopes. The problem of zonotopal tiling, i.e., paving a zonotope by tiles (sub-zonotopes) without gaps and overlaps, is an important topic in combinatorics and topology \cite{bjorner1999oriented,ziegler2012lectures}. In the realm of zonotopal tiling, Bohne-Dress theorem \cite{richter1994zonotopal} plays a crucial role by proving that a tiling of a zonotope can be uniquely represented by a collection of sign vectors or oriented matroid. Inspired by this theorem, \cite{kabi2020synthesizing} developed a tiling method  by enumerating the vertices of the tiles as sign vectors of the so-called hyperplane arrangement \cite{mcmullen1971zonotopes} corresponding to a zonotope. However, in this paper we provide a novel and more accessible method for constructing a zonotopal tiling, which has better computational complexity.
% Due to some favorable properties such as closure under linear maps and Minkowski sum, they find extensive applications in formal verification including reachability analysis \cite{girard2005reachability,althoff2010computing}, invariant 
% synthesis \cite{kabi2020synthesizing} and fault detection \cite{wang2018robust}.

% To mitigate wrapping effect \cite{neumaier1993wrapping} and enhance computed results, it is a common way to split a zonotope into smaller sub-zonotopes during computation. 
% In the works \cite{althoff2008reachability,wan2009numerical}, they split a zonotope by bisecting it along one of its generator. However, the sub-zonotopes split by this way often have overlap parts, resulting in loss of precision and heavy computation burden. Hence, there is a pressing need for methods that split a zonotope into non-overlapping sub-zonotopes. The problem of zonotopal tiling, i.e., paving a zonotope by tiles (sub-zonotopes) without gaps and overlaps, is an important topic in combinatorics and topology \cite{bjorner1999oriented,ziegler2012lectures}.
%Besides Minkowski sum of lines segments or linear projection of a cube, one can characterize a zonotope by a polar dual of hyperplane arrangement \cite{mcmullen1971zonotopes}. Utilizing the dual relationship between a zonotope and its corresponding hyperplane arrangement, 
% In the realm of zonotopal tiling, Bohne-Dress theorem \cite{richter1994zonotopal} plays a crucial role by proving that a tiling of a zonotope can be uniquely represented by a collection of sign vectors or oriented matroid. Inspired by this theorem, \cite{kabi2020synthesizing} developed a tiling method  by enumerating the vertices of the tiles as sign vectors of the so-called hyperplane arrangement \cite{mcmullen1971zonotopes} corresponding to a zonotope. However, in this paper we provide a novel and more accessible method for constructing a zonotopal tiling. This approach is not only easier to comprehend but also simpler to implement, achieved through two innovative data structures: the boundary matrix and the tiling matrix.
%our novel tiling algorithm proposed is implemented in different way via recursively decomposing the pre-iteration zonotope into a collection of sub-zonotopes and a singer zonotope with a generator removed. Each iteration executes a movement of one-sided facets of pre-iteration zonotope which is encoded by two new data structures, i.e., boundary matrix and tiling matrix.  
%enhanced the set-boundary reachability method using polynomial zonotopes, which 

%applies polynomial zonotope, a non-convex set, in this framework instead of polytopes in \cite{xue2016under}. Since the utilization of non-convex sets, the inner-approximations computed by \cite{kochdumper2020computing}  have better precision than previous methods. However, they only support the initial set with the interval form, which brings some conservativeness in the case having more complex initial set. Since the absence of the iteration, they can not compute inner-approximations at long time instance. 


%raises a theorem related to boundary analysis: the boundary of the reachable set of initial set at time instant $t$ is equal to the reachable set of the boundary of initial set at time instant $t$. Based on this theorem, \cite{xue2016under} propose a framework to compute inner-approximations: firstly the over-approximation of boundary is computed, and then contract the over-approximation of reachable set to obtain an inner-approximation candidate until there is no intersection between this candidate and the over-approximation of boundary.







%\textcolor{red}{The exact boundaries of polytopes and polynomial zonotopes are hard to obtain, in \cite{xue2016under} and \cite{kochdumper2020computing} they use over-approximation of the boundaries instead of the exact ones, which will reduce the precision of the computation.} 
%\color{red}
%In this work, we compute inner-approximations with the same pipeline as in \cite{xue2016under} but propagating zonotope boundaries exactly to weaken the wrapping-effect and thus improve the performance of computing inner-approximations.
%\color{black}

The remainder of this paper is organized as follows. The inner-approximate reachability problem of interest is presented in Sect. \ref{preliminaries}. Then, we elucidate our reachability computational approach in Sect. \ref{method} and evaluate it in Sect. \ref{experiment}. Finally, we summarize the paper in Sect. \ref{conclusion}.


 

%There are a few works on computing inner-approximation of reachable sets for linear systems, e.g. \cite{maidens2013lagrangian}, \cite{girard2006efficient}, \cite{hamadeh2008reachability}, \cite{kurzhanski2000ellipsoidal}. However, these works can not be straightforward extended to compute inner-approximation of reachable sets for nonlinear systems. Recently, some methods have been developed for nonlinear systems.

%Several methods compute level-sets to represent inner-approximations on Hamilton-Jacobi framework, e.g. \cite{li2018safe}, \cite{mitchell2005time}. \textcolor{red}{Since the utilization of Hamilton-Jacobi framework, they all suffer the curse of the dimension.} For polynomial dynamical systems, sum-of squares (SOS) programming methods are proposed to obtain inner approximation of reachable sets in  \cite{wang2013polynomial}, \cite{korda2013inner}, \cite{xue2018under}, \cite{xue2019inner}. These SOS based method compute inner-approximations represented by level-sets, which are more expressive since its non-convex representations. However, the present status of SOS solvers is not so advanced. In some cases the results of these solvers are unreliable caused by the numerical problems. Moreover, these methods are not suitable for high-dimensional systems since the size of semi-define program grows rapidly with the dimension of system.


%We also apply the framework in \cite{xue2016under}, however, with the novel techniques proposed in this paper, the efficiency and precision have been improved much more than \cite{xue2016under} and \cite{kochdumper2020computing}.

%Although the computed  inner-approximations of  projection are useful for some verification tasks, they may not able to handle the more complex verification issues. \textcolor{cyan}{Moreover, our approach can accomplish more complex verification problem such as determine whether a point lies in the inner-approximation of the reachable set while \cite{goubault2017forward} can't since we compute the inner-approximation of the whole reachable set.}


%There are some methods computing inner-approximations using interval arithmetic, e.g. \cite{goldsztejn2010inner}, \cite{olivier2013general}, \cite{goubault2014inner}. These interval methods introduce more conservativeness which will make the inner-approximation less precision.
%\cite{goubault2017forward} proposed an efficient approach to compute the inner-approximations of  projection onto the coordinate axes for autonomous nonlinear systems. They extended this method for systems with uncertain inputs in \cite{goubault2019inner}. Although the inner-approximations of  projection are often useful for simple verification tasks, they may not able to handle the more complex verification issues. 
